Optimal Reactive Operation of General Topology Supply Chain and Manufacturing Networks under Disruptions

Supply and manufacturing networks in the chemical industry involve diverse processing steps across different locations, rendering their operation vulnerable to disruptions from unplanned events. Optimal responses should consider factors such as product allocation, delayed shipments, and price renegotiation , among other factors. In such context, we propose a multiperiod mixed-integer linear programming model that integrates production, scheduling, shipping, and order management to minimize the financial impact of such disruptions. The model accommodates arbitrary supply chain topologies and incorporates various disruption scenarios, offering adaptability to real-world complexities. A case study from the chemical industry demonstrates the scalability of the model under finer time discretization and explores the influence of disruption types and order management costs on optimal schedules. This approach provides a tractable, adaptable framework for developing responsive operational plans in supply chain and manufacturing networks under uncertainty.

==> bibliography.tex <==
@book{bynum2021pyomo,
title={{Pyomo--optimization modeling in python}},
author={Bynum, Michael L. and Hackebeil, Gabriel A. and Hart, William E. and Laird, Carl D. and Nicholson, Bethany L. and Siirola, John D. and Watson, Jean-Paul and Woodruff, David L.},
edition={Third},
volume={67},
year={2021},
publisher={Springer Science \& Business Media}
}
@article{grossmann2013systematic,
  title={{Systematic modeling of discrete-continuous optimization models through generalized disjunctive programming}},
  author={Grossmann, Ignacio E and Trespalacios, Francisco},
  journal={AIChE Journal},
  volume={59},
  number={9},
  pages={3276--3295},
  year={2013},
  publisher={Wiley Online Library}
}
@article{raman1994modelling,
  title={{Modelling and computational techniques for logic based integer programming}},
  author={Raman, Ramesh and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={18},
  number={7},
  pages={563--578},
  year={1994},
  publisher={Elsevier}
}
@article{lee2000new,
  title={{New algorithms for nonlinear generalized disjunctive programming}},
  author={Lee, Sangbum and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={24},
  number={9-10},
  pages={2125--2141},
  year={2000},
  publisher={Elsevier}
}
@article{sawaya2005cutting,
  title={{A cutting plane method for solving linear generalized disjunctive programming problems}},
  author={Sawaya, Nicolas W and Grossmann, Ignacio E},
  journal={Computers \& chemical engineering},
  volume={29},
  number={9},
  pages={1891--1913},
  year={2005},
  publisher={Elsevier}
}
@article{turkay1996logic,
  title={{Logic-based MINLP algorithms for the optimal synthesis of process networks}},
  author={T{\"u}rkay, Metin and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={20},
  number={8},
  pages={959--978},
  year={1996},
  publisher={Elsevier}
}
@article{grossmann2002review,
  title={{Review of nonlinear mixed-integer and disjunctive programming techniques}},
  author={Grossmann, Ignacio E},
  journal={Optimization and engineering},
  volume={3},
  pages={227--252},
  year={2002},
  publisher={Springer}
}
@inproceedings{chong2009model,
  title={{Model-based control of multi-unit systems under partial shutdown conditions}},
  author={Chong, Zhiwen and Swartz, Christopher LE},
  booktitle={2009 American Control Conference},
  pages={160--165},
  year={2009},
  organization={IEEE}
}
@article{perea2003model,
  title={{A model predictive control strategy for supply chain optimization}},
  author={Perea-Lopez, Edgar and Ydstie, B Erik and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={27},
  number={8-9},
  pages={1201--1218},
  year={2003},
  publisher={Elsevier}
}
@article{kim2005adaptive,
  title={{Adaptive inventory control models for supply chain management}},
  author={Kim, CO and Jun, J and Baek, JK and Smith, RL and Kim, Yeong-Dae},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={26},
  number={9},
  pages={1184--1192},
  year={2005},
  publisher={Springer}
}
@book{snyder2019fundamentals,
  title={{Fundamentals of Supply Chain Theory}},
  author={Snyder, Lawrence V and Shen, Zuo-Jun Max},
  year={2019},
  publisher={John Wiley \& Sons}
}
@inproceedings{sharda2008discrete,
  title={{A discrete event simulation model for reliability modeling of a chemical plant}},
  author={Sharda, Bikram and Bury, Scott J},
  booktitle={2008 Winter Simulation Conference},
  pages={1736--1740},
  year={2008},
  organization={IEEE}
}
@incollection{perez2021digital,
  title={{A Digital Twin Framework for Business Transactional Processes in Supply Chains}},
  author={Perez, Hector D and Amaran, Satyajith and Erisen, Esra and Wassick, John M and Grossmann, Ignacio E},
  booktitle={Computer Aided Chemical Engineering},
  volume={50},
  pages={1755--1760},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{deleris2005risk,
  title={{Risk management in supply networks using Monte-Carlo simulation}},
  author={Deleris, L{\'e}a A and Erhun, Feryal},
  booktitle={Proceedings of the Winter Simulation Conference, 2005.},
  pages={7--pp},
  year={2005},
  organization={IEEE}
}
@inproceedings{schmitt2009quantifying,
  title={{Quantifying supply chain disruption risk using Monte Carlo and discrete-event simulation}},
  author={Schmitt, Amanda J and Singh, Mahender},
  booktitle={Proceedings of the 2009 winter simulation conference (WSC)},
  pages={1237--1248},
  year={2009},
  organization={IEEE}
}
@article{garcia2014design,
  title={{Design of resilient supply chains with risk of facility disruptions}},
  author={Garcia-Herreros, Pablo and Wassick, John M and Grossmann, Ignacio E},
  journal={Industrial \& Engineering Chemistry Research},
  volume={53},
  number={44},
  pages={17240--17251},
  year={2014},
  publisher={ACS Publications}
}
@article{simpson1958process,
  title={{In-process inventories}},
  author={Simpson Jr, Kenneth F},
  journal={Operations Research},
  volume={6},
  number={6},
  pages={863--873},
  year={1958},
  publisher={INFORMS}
}
@article{graves2000optimizing,
  title={{Optimizing strategic safety stock placement in supply chains}},
  author={Graves, Stephen C and Willems, Sean P},
  journal={Manufacturing \& Service Operations Management},
  volume={2},
  number={1},
  pages={68--83},
  year={2000},
  publisher={INFORMS}
}
@article{bossert2007periodic,
  title={{A periodic-review modeling approach for guaranteed service supply chains}},
  author={Bossert, John M and Willems, Sean P},
  journal={Interfaces},
  volume={37},
  number={5},
  pages={420--436},
  year={2007},
  publisher={INFORMS}
}
@unpublished{achkarinforms,
title= {{Integrated Guaranteed Service Approach for Multi-echelon Inventory Optimization}},
author = {Achkar, Victoria G and Brunaud, Braulio and Musa, Rami and Mendez, Carlos A and Grossmann, Ignacio E},
year = {2021},
note= {INFORMS Annual Meeting, Anaheim, CA},
}
@article{balasubramanian2004approximation,
  title={{Approximation to multistage stochastic optimization in multiperiod batch plant scheduling under demand uncertainty}},
  author={Balasubramanian, J and Grossmann, IE},
  journal={Industrial \& engineering chemistry research},
  volume={43},
  number={14},
  pages={3695--3713},
  year={2004},
  publisher={ACS Publications}
}

@article{grossmann2012advances,
  title={{Advances in mathematical programming models for enterprise-wide optimization}},
  author={Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={47},
  pages={2--18},
  year={2012},
  publisher={Elsevier}
}
@article{shah2004pharmaceutical,
  title={{Pharmaceutical supply chains: key issues and strategies for optimisation}},
  author={Shah, Nilay},
  journal={Computers \& chemical engineering},
  volume={28},
  number={6-7},
  pages={929--941},
  year={2004},
  publisher={Elsevier}
}
@article{floudas2004continuous,
  title={{Continuous-time versus discrete-time approaches for scheduling of chemical processes: a review}},
  author={Floudas, Christodoulos A and Lin, Xiaoxia},
  journal={Computers \& Chemical Engineering},
  volume={28},
  number={11},
  pages={2109--2129},
  year={2004},
  publisher={Elsevier}
}
@article{mendez2006state,
  title={{State-of-the-art review of optimization methods for short-term scheduling of batch processes}},
  author={M{\'e}ndez, Carlos A and Cerd{\'a}, Jaime and Grossmann, Ignacio E and Harjunkoski, Iiro and Fahl, Marco},
  journal={Computers \& chemical engineering},
  volume={30},
  number={6-7},
  pages={913--946},
  year={2006},
  publisher={Elsevier}
}
@misc{gurobi,
  author = {{Gurobi Optimization, LLC}},
  title = {{Gurobi Optimizer Reference Manual}},
  year = 2022,
  url = "https://www.gurobi.com"
}
@article{owen1998strategic,
  title={{Strategic facility location: A review}},
  author={Owen, Susan Hesse and Daskin, Mark S},
  journal={European Journal of Operational Research},
  volume={111},
  number={3},
  pages={423--447},
  year={1998},
  publisher={Elsevier}
}
@article{braekers2016vehicle,
  title={{The vehicle routing problem: State of the art classification and review}},
  author={Braekers, Kris and Ramaekers, Katrien and Van Nieuwenhuyse, Inneke},
  journal={Computers \& Industrial Engineering},
  volume={99},
  pages={300--313},
  year={2016},
  publisher={Elsevier}
}
@article{shang2003newsvendor,
  title={{Newsvendor bounds and heuristic for optimal policies in serial supply chains}},
  author={Shang, Kevin H and Song, Jing-Sheng},
  journal={Management Science},
  volume={49},
  number={5},
  pages={618--638},
  year={2003},
  publisher={INFORMS}
}
@article{clark1960optimal,
  title={{Optimal policies for a multi-echelon inventory problem}},
  author={Clark, Andrew J and Scarf, Herbert},
  journal={Management science},
  volume={6},
  number={4},
  pages={475--490},
  year={1960},
  publisher={INFORMS}
}
@article{chen1994evaluating,
  title={{Evaluating echelon stock (R, nQ) policies in serial production/inventory systems with stochastic demand}},
  author={Chen, Fangruo and Zheng, Yu-Sheng},
  journal={Management Science},
  volume={40},
  number={10},
  pages={1262--1275},
  year={1994},
  publisher={INFORMS}
}
@article{rosling1989optimal,
  title={{Optimal inventory policies for assembly systems under random demands}},
  author={Rosling, Kaj},
  journal={Operations Research},
  volume={37},
  number={4},
  pages={565--579},
  year={1989},
  publisher={INFORMS}
}
@article{schmitt2015centralization,
  title={{Centralization versus decentralization: Risk pooling, risk diversification, and supply chain disruptions}},
  author={Schmitt, Amanda J and Sun, Siyuan Anthony and Snyder, Lawrence V and Shen, Zuo-Jun Max},
  journal={Omega},
  volume={52},
  pages={201--212},
  year={2015},
  publisher={Elsevier}
}
@article{sherbrooke1968metric,
  title={{METRIC: A multi-echelon technique for recoverable item control}},
  author={Sherbrooke, Craig C},
  journal={Operations Research},
  volume={16},
  number={1},
  pages={122--141},
  year={1968},
  publisher={INFORMS}
}
@article{rong2017heuristics,
  title={{Heuristics for base-stock levels in multi-echelon distribution networks}},
  author={Rong, Ying and Atan, Z{\"u}mb{\"u}l and Snyder, Lawrence V},
  journal={Production and Operations Management},
  volume={26},
  number={9},
  pages={1760--1777},
  year={2017},
  publisher={Wiley Online Library}
}
@book{wolsey1999integer,
  title={{Integer and combinatorial optimization}},
  author={Wolsey, Laurence A and Nemhauser, George L},
  volume={55},
  year={1999},
  publisher={John Wiley \& Sons}
}
@article{you2013multicut,
  title={{Multicut Benders decomposition algorithm for process supply chain planning under uncertainty}},
  author={You, Fengqi and Grossmann, Ignacio E},
  journal={Annals of Operations Research},
  volume={210},
  number={1},
  pages={191--211},
  year={2013},
  publisher={Springer}
}

@article{mitchell2021engineering,
  title={{Engineering precision nanoparticles for drug delivery}},
  author={Mitchell, Michael J and Billingsley, Margaret M and Haley, Rebecca M and Wechsler, Marissa E and Peppas, Nicholas A and Langer, Robert},
  journal={Nature Reviews Drug Discovery},
  volume={20},
  number={2},
  pages={101--124},
  year={2021},
  publisher={Nature Publishing Group UK London}
}
@article{wamble2022optimal,
  title={{Optimal diafiltration membrane cascades enable green recycling of spent lithium-ion batteries}},
  author={Wamble, Noah P and Eugene, Elvis A and Phillip, William A and Dowling, Alexander W},
  journal={ACS Sustainable Chemistry \& Engineering},
  volume={10},
  number={37},
  pages={12207--12225},
  year={2022},
  publisher={ACS Publications}
}
@article{trespalacios2015improved,
  title={{Improved Big-M reformulation for generalized disjunctive programs}},
  author={Trespalacios, Francisco and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={76},
  pages={98--103},
  year={2015},
  publisher={Elsevier}
}
@article{lima2011long,
  title={{Long-term scheduling of a single-unit multi-product continuous process to manufacture high performance glass}},
  author={Lima, Ricardo M and Grossmann, Ignacio E and Jiao, Yu},
  journal={Computers \& Chemical Engineering},
  volume={35},
  number={3},
  pages={554--574},
  year={2011},
  publisher={Elsevier}
}
@article{subramanian2013integration,
  title={{Integration of control theory and scheduling methods for supply chain management}},
  author={Subramanian, Kaushik and Rawlings, James B and Maravelias, Christos T and Flores-Cerrillo, Jesus and Megan, Lawrence},
  journal={Computers \& Chemical Engineering},
  volume={51},
  pages={4--20},
  year={2013},
  publisher={Elsevier}
}
@book{rawlings2017model,
  title={Model predictive control: Theory, computation, and design},
  author={Rawlings, James Blake and Mayne, David Q and Diehl, Moritz and others},
  volume={2},
  year={2017},
  publisher={Nob Hill Publishing Madison, WI}
}
@article{ceccon2022omlt,
  title={{OMLT: Optimization \& machine learning toolkit}},
  author={Ceccon, Francesco and Jalving, Jordan and Haddad, Joshua and Thebelt, Alexander and Tsay, Calvin and Laird, Carl D and Misener, Ruth},
  journal={The Journal of Machine Learning Research},
  volume={23},
  number={1},
  pages={15829--15836},
  year={2022},
  publisher={JMLRORG}
}
@article{balas1985disjunctive,
  title={{Disjunctive programming and a hierarchy of relaxations for discrete optimization problems}},
  author={Balas, Egon},
  journal={SIAM Journal on Algebraic Discrete Methods},
  volume={6},
  number={3},
  pages={466--486},
  year={1985},
  publisher={SIAM}
}
@incollection{perez2023modeling,
  title={{Modeling hierarchical systems via nested generalized disjunctive programming}},
  author={Perez, Hector D and Grossmann, Ignacio E},
  booktitle={Computer Aided Chemical Engineering},
  volume={52},
  pages={1373--1378},
  year={2023},
  publisher={Elsevier}
}
@article{maravelias2003new,
  title={{New general continuous-time State- Task network formulation for short-term scheduling of multipurpose batch plants}},
  author={Maravelias, Christos T and Grossmann, Ignacio E},
  journal={Industrial \& Engineering Chemistry Research},
  volume={42},
  number={13},
  pages={3056--3074},
  year={2003},
  publisher={ACS Publications}
}
@article{kondili1993general,
  title={{A general algorithm for short-term scheduling of batch operations—I. MILP formulation}},
  author={Kondili, Emilia and Pantelides, Constantinos C and Sargent, Roger WH},
  journal={Computers \& Chemical Engineering},
  volume={17},
  number={2},
  pages={211--227},
  year={1993},
  publisher={Elsevier}
}
@article{bugert2018supply,
  title={{Supply chain disruption models: A critical review}},
  author={Bugert, Niels and Lasch, Rainer},
  journal={Logistics Research},
  volume={11},
  number={5},
  pages={1--35},
  year={2018},
  publisher={Bremen: Bundesvereinigung Logistik (BVL)}
}
@article{shekarian2021integrative,
  title={{An integrative approach to supply chain disruption risk and resilience management: A literature review}},
  author={Shekarian, Mansoor and Mellat Parast, Mahour},
  journal={International Journal of Logistics Research and Applications},
  volume={24},
  number={5},
  pages={427--455},
  year={2021},
  publisher={Taylor \& Francis}
}
@book{sawik2020supply,
  title={{Supply chain disruption management}},
  author={Sawik, Tadeusz and others},
  year={2020},
  publisher={Springer}
}
@article{ivanov2017literature,
  title={{Literature review on disruption recovery in the supply chain}},
  author={Ivanov, Dmitry and Dolgui, Alexandre and Sokolov, Boris and Ivanova, Marina},
  journal={International Journal of Production Research},
  volume={55},
  number={20},
  pages={6158--6174},
  year={2017},
  publisher={Taylor \& Francis}
}
@article{snyder2016or,
  title={{OR/MS models for supply chain disruptions: A review}},
  author={Snyder, Lawrence V and Atan, Z{\"u}mb{\"u}l and Peng, Peng and Rong, Ying and Schmitt, Amanda J and Sinsoysal, Burcu},
  journal={IIE Transactions},
  volume={48},
  number={2},
  pages={89--109},
  year={2016},
  publisher={Taylor \& Francis}
}
@article{katsaliaki2021supply,
  title={{Supply chain disruptions and resilience: A major review and future research agenda}},
  author={Katsaliaki, Korina and Galetsi, Panagiota and Kumar, Sameer},
  journal={Annals of Operations Research},
  pages={1--38},
  year={2021},
  publisher={Springer}
}
@article{etemadi2021supply,
  title={{Supply chain disruption risk management with blockchain: A dynamic literature review}},
  author={Etemadi, Niloofar and Borbon-Galvez, Yari and Strozzi, Fernanda and Etemadi, Tahereh},
  journal={Information},
  volume={12},
  number={2},
  pages={70},
  year={2021},
  publisher={MDPI}
}
@article{xu2020disruption,
  title={{Disruption risks in supply chain management: a literature review based on bibliometric analysis}},
  author={Xu, Song and Zhang, Xiaotong and Feng, Lipan and Yang, Wenting},
  journal={International Journal of Production Research},
  volume={58},
  number={11},
  pages={3508--3526},
  year={2020},
  publisher={Taylor \& Francis}
}
@article{dolgui2021ripple,
  title={{Ripple effect and supply chain disruption management: new trends and research directions}},
  author={Dolgui, Alexandre and Ivanov, Dmitry},
  journal={International Journal of Production Research},
  volume={59},
  number={1},
  pages={102--109},
  year={2021},
  publisher={Taylor \& Francis}
}
@article{moosavi2022supply,
  title={{Supply chain disruption during the COVID-19 pandemic: Recognizing potential disruption management strategies}},
  author={Moosavi, Javid and Fathollahi-Fard, Amir M and Dulebenets, Maxim A},
  journal={International Journal of Disaster Risk Reduction},
  volume={75},
  pages={102983},
  year={2022},
  publisher={Elsevier}
}
@article{tomlin2006value,
  title={{On the value of mitigation and contingency strategies for managing supply chain disruption risks}},
  author={Tomlin, Brian},
  journal={Management science},
  volume={52},
  number={5},
  pages={639--657},
  year={2006},
  publisher={INFORMS}
}
@article{schutz2011impact,
  title={{The impact of flexibility on operational supply chain planning}},
  author={Sch{\"u}tz, Peter and Tomasgard, Asgeir},
  journal={International Journal of Production Economics},
  volume={134},
  number={2},
  pages={300--311},
  year={2011},
  publisher={Elsevier}
}
@article{ivanov2020predicting,
  title={{Predicting the impacts of epidemic outbreaks on global supply chains: A simulation-based analysis on the coronavirus outbreak (COVID-19/SARS-CoV-2) case}},
  author={Ivanov, Dmitry},
  journal={Transportation Research Part E: Logistics and Transportation Review},
  volume={136},
  pages={101922},
  year={2020},
  publisher={Elsevier}
}
@article{ribeiro2018supply,
  title={{Supply Chain Resilience: Definitions and quantitative modelling approaches--A literature review}},
  author={Ribeiro, Joao Pires and Barbosa-Povoa, Ana},
  journal={Computers \& Industrial Engineering},
  volume={115},
  pages={109--122},
  year={2018},
  publisher={Elsevier}
}
@article{you2008design,
  title={{Design of responsive supply chains under demand uncertainty}},
  author={You, Fengqi and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={32},
  number={12},
  pages={3090--3111},
  year={2008},
  publisher={Elsevier}
}
@article{you2009risk,
  title={{Risk management for a global supply chain planning under uncertainty: models and algorithms}},
  author={You, Fengqi and Wassick, John M and Grossmann, Ignacio E},
  journal={AIChE Journal},
  volume={55},
  number={4},
  pages={931--946},
  year={2009},
  publisher={Wiley Online Library}
}
@article{elleuch2016resilience,
  title={{Resilience and vulnerability in supply chain: Literature review}},
  author={Elleuch, Hatem and Dafaoui, E and Elmhamedi, A and Chabchoub, H},
  journal={IFAC-PapersOnLine},
  volume={49},
  number={12},
  pages={1448--1453},
  year={2016},
  publisher={Elsevier}
}
@article{kamalahmadi2016review,
  title={{A review of the literature on the principles of enterprise and supply chain resilience: Major findings and directions for future research}},
  author={Kamalahmadi, Masoud and Parast, Mahour Mellat},
  journal={International Journal of Production Economics},
  volume={171},
  pages={116--133},
  year={2016},
  publisher={Elsevier}
}
@article{cardoso2015resilience,
  title={{Resilience metrics in the assessment of complex supply-chains performance operating under demand uncertainty}},
  author={Cardoso, S{\'o}nia R and Barbosa-P{\'o}voa, Ana Paula and Relvas, Susana and Novais, Augusto Q},
  journal={Omega},
  volume={56},
  pages={53--73},
  year={2015},
  publisher={Elsevier}
}
@article{adenso2012impact,
  title={{The impact of supply network characteristics on reliability}},
  author={Adenso-Diaz, Belarmino and Mena, Carlos and Garc{\'\i}a-Carbajal, Santiago and Liechty, Merrill},
  journal={Supply Chain Management: An International Journal},
  volume={17},
  number={3},
  pages={263--276},
  year={2012},
  publisher={Emerald Group Publishing Limited}
}
@article{azevedo2016larg,
  title={{LARG index: A benchmarking tool for improving the leanness, agility, resilience and greenness of the automotive supply chain}},
  author={Azevedo, Susana Garrido and Carvalho, Helena and Cruz-Machado, V},
  journal={Benchmarking: An International Journal},
  volume={23},
  number={6},
  pages={1472--1499},
  year={2016},
  publisher={Emerald Group Publishing Limited}
}
@article{munoz2015quantification,
  title={{On the quantification of operational supply chain resilience}},
  author={Munoz, Albert and Dunbar, Michelle},
  journal={International Journal of Production Research},
  volume={53},
  number={22},
  pages={6736--6751},
  year={2015},
  publisher={Taylor \& Francis}
}
@article{dixit2016performance,
  title={{Performance measures based optimization of supply chain network resilience: A NSGA-II+ Co-Kriging approach}},
  author={Dixit, Vijaya and Seshadrinath, Navaneeth and Tiwari, MK},
  journal={Computers \& Industrial Engineering},
  volume={93},
  pages={205--214},
  year={2016},
  publisher={Elsevier}
}
@article{glasserman1995sensitivity,
  title={{Sensitivity analysis for base-stock levels in multiechelon production-inventory systems}},
  author={Glasserman, Paul and Tayur, Sridhar},
  journal={Management Science},
  volume={41},
  number={2},
  pages={263--281},
  year={1995},
  publisher={INFORMS}
}
@article{snyder2006facility,
  title={{Facility location under uncertainty: A review}},
  author={Snyder, Lawrence V},
  journal={IIE Transactions},
  volume={38},
  number={7},
  pages={547--564},
  year={2006},
  publisher={Taylor \& Francis}
}
@article{melo2009facility,
  title={{Facility location and supply chain management--A review}},
  author={Melo, M Teresa and Nickel, Stefan and Saldanha-Da-Gama, Francisco},
  journal={European journal of operational research},
  volume={196},
  number={2},
  pages={401--412},
  year={2009},
  publisher={Elsevier}
}
@article{snyder2005reliability,
  title={{Reliability models for facility location: the expected failure cost case}},
  author={Snyder, Lawrence V and Daskin, Mark S},
  journal={Transportation Science},
  volume={39},
  number={3},
  pages={400--416},
  year={2005},
  publisher={INFORMS}
}
@article{tsiakis2001design,
  title={{Design of multi-echelon supply chain networks under demand uncertainty}},
  author={Tsiakis, Panagiotis and Shah, Nilay and Pantelides, Constantinos C},
  journal={Industrial \& Engineering Chemistry Research},
  volume={40},
  number={16},
  pages={3585--3604},
  year={2001},
  publisher={ACS Publications}
}
@article{you2008mixed,
  title={{Mixed-integer nonlinear programming models and algorithms for large-scale supply chain design with stochastic inventory management}},
  author={You, Fengqi and Grossmann, Ignacio E},
  journal={Industrial \& Engineering Chemistry Research},
  volume={47},
  number={20},
  pages={7802--7817},
  year={2008},
  publisher={ACS Publications}
}
@article{chen1989effects,
  title={{Effects of centralization on expected costs in a multi-location newsboy problem}},
  author={Chen, Miao-Sheng and Lin, Chin-Tsai},
  journal={Journal of the Operational Research Society},
  volume={40},
  pages={597--602},
  year={1989},
  publisher={Springer}
}
@article{snyder2006supply,
  title={{Supply and demand uncertainty in multi-echelon supply chains}},
  author={Snyder, Lawrence V and Shen, Zuo-Jun Max},
  journal={Submitted for publication, Lehigh University},
  volume={15},
  year={2006},
  publisher={Citeseer}
}
@article{lim2010facility,
  title={{A facility reliability problem: Formulation, properties, and algorithm}},
  author={Lim, Michael and Daskin, Mark S and Bassamboo, Achal and Chopra, Sunil},
  journal={Naval Research Logistics (NRL)},
  volume={57},
  number={1},
  pages={58--70},
  year={2010},
  publisher={Wiley Online Library}
}
@article{shen2011reliable,
  title={{The reliable facility location problem: Formulations, heuristics, and approximation algorithms}},
  author={Shen, Zuo-Jun Max and Zhan, Roger Lezhou and Zhang, Jiawei},
  journal={INFORMS Journal on Computing},
  volume={23},
  number={3},
  pages={470--482},
  year={2011},
  publisher={INFORMS}
}
@article{cui2010reliable,
  title={{Reliable facility location design under the risk of disruptions}},
  author={Cui, Tingting and Ouyang, Yanfeng and Shen, Zuo-Jun Max},
  journal={Operations Research},
  volume={58},
  number={4-part-1},
  pages={998--1011},
  year={2010},
  publisher={INFORMS}
}
@article{li2010continuum,
  title={{A continuum approximation approach to reliable facility location design under correlated probabilistic disruptions}},
  author={Li, Xiaopeng and Ouyang, Yanfeng},
  journal={Transportation Research Part B: Methodological},
  volume={44},
  number={4},
  pages={535--548},
  year={2010},
  publisher={Elsevier}
}
@article{santoso2005stochastic,
  title={{A stochastic programming approach for supply chain network design under uncertainty}},
  author={Santoso, Tjendera and Ahmed, Shabbir and Goetschalckx, Marc and Shapiro, Alexander},
  journal={European Journal of Operational Research},
  volume={167},
  number={1},
  pages={96--115},
  year={2005},
  publisher={Elsevier}
}
@article{klibi2012scenario,
  title={{Scenario-based supply chain network risk modeling}},
  author={Klibi, Walid and Martel, Alain},
  journal={European Journal of Operational Research},
  volume={223},
  number={3},
  pages={644--658},
  year={2012},
  publisher={Elsevier}
}
@article{klibi2010design,
  title={{The design of robust value-creating supply chain networks: A critical review}},
  author={Klibi, Walid and Martel, Alain and Guitouni, Adel},
  journal={European Journal of Operational Research},
  volume={203},
  number={2},
  pages={283--293},
  year={2010},
  publisher={Elsevier}
}
@article{manuj2009improving,
  title={{Improving the rigor of discrete-event simulation in logistics and supply chain research}},
  author={Manuj, Ila and Mentzer, John T and Bowers, Melissa R},
  journal={International Journal of Physical Distribution \& Logistics Management},
  volume={39},
  number={3},
  pages={172--201},
  year={2009},
  publisher={Emerald Group Publishing Limited}
}
@article{hajian2022supply,
  title={{Supply Chain Resilience Analysis Considering Disruption in the Natural Stone Industry Using a Discrete-Event Simulation Approach}},
  author={Hajian Heidary, Mojtaba and Mirzaaliyan, Maede},
  journal={Journal of Industrial Management Perspective},
  volume={12},
  number={4, Winter 2023},
  pages={97--129},
  year={2022},
  publisher={Shahid Beheshti University}
}
@article{kogler2018discrete,
  title={{Discrete event simulation of multimodal and unimodal transportation in the wood supply chain: a literature review}},
  author={Kogler, Christoph and Rauch, Peter},
  journal={Silva Fennica},
  volume={52},
  number={4},
  year={2018}
}
@article{abideen2021improving,
  title={{Improving the performance of a Malaysian pharmaceutical warehouse supply chain by integrating value stream mapping and discrete event simulation}},
  author={Abideen, Ahmed and Mohamad, Fazeeda Binti},
  journal={Journal of Modelling in Management},
  volume={16},
  number={1},
  pages={70--102},
  year={2021},
  publisher={Emerald Publishing Limited}
}
@article{prasoon2017replenishment,
  title={{Replenishment policy in a two-echelon supply chain: An analysis using discrete-event simulation}},
  author={Prasoon, Ruchir and Agarwal, Maulik and Kumar, Ajith},
  journal={International Journal of Business Analytics and Intelligence},
  volume={5},
  number={2},
  pages={37},
  year={2017},
  publisher={Publishing India Group}
}
@article{vidalakis2013demand,
  title={{Demand uncertainty in construction supply chains: a discrete event simulation study}},
  author={Vidalakis, Christos and Tookey, John E and Sommerville, James},
  journal={Journal of the Operational Research Society},
  volume={64},
  number={8},
  pages={1194--1204},
  year={2013},
  publisher={Taylor \& Francis}
}
@article{jha2023multi,
  title={{A multi-period discrete event simulation model for comparing synchronous and asynchronous facility reopening in global supply chains affected by disruption}},
  author={Jha, Harshit and Mohan, Usha},
  journal={Supply Chain Analytics},
  volume={2},
  pages={100010},
  year={2023},
  publisher={Elsevier}
}
@article{perez2022digital,
  title={{A digital twin framework for online optimization of supply chain business processes}},
  author={Perez, Hector D and Wassick, John M and Grossmann, Ignacio E},
  journal={Computers \& Chemical Engineering},
  volume={166},
  pages={107972},
  year={2022},
  publisher={Elsevier}
}
@incollection{goldsman2015discrete,
  title={{Discrete-event simulation}},
  author={Goldsman, David and Goldsman, Paul},
  booktitle={Modeling and Simulation in the Systems Engineering Life Cycle: Core Concepts and Accompanying Lectures},
  pages={103--109},
  year={2015},
  publisher={Springer}
}
@article{badejo2022mathematical,
  title={{Mathematical programming approach to optimize tactical and operational supply chain decisions under disruptions}},
  author={Badejo, Oluwadare and Ierapetritou, Marianthi},
  journal={Industrial \& Engineering Chemistry Research},
  volume={61},
  number={45},
  pages={16747--16763},
  year={2022},
  publisher={ACS Publications}
}
@article{pistikopoulos2021process,
  title={{Process systems engineering--the generation next?}},
  author={Pistikopoulos, Efstratios N and Barbosa-Povoa, Ana and Lee, Jay H and Misener, Ruth and Mitsos, Alexander and Reklaitis, Gintaras V and Venkatasubramanian, Venkat and You, Fengqi and Gani, Rafiqul},
  journal={Computers \& Chemical Engineering},
  volume={147},
  pages={107252},
  year={2021},
  publisher={Elsevier}
}
@article{garcia2015supply,
  title={{Supply chain design and optimization: Challenges and opportunities}},
  author={Garcia, Daniel J and You, Fengqi},
  journal={Computers \& Chemical Engineering},
  volume={81},
  pages={153--170},
  year={2015},
  publisher={Elsevier}
}
@article{shah2005process,
  title={{Process industry supply chains: Advances and challenges}},
  author={Shah, Nilay},
  journal={Computers \& Chemical Engineering},
  volume={29},
  number={6},
  pages={1225--1235},
  year={2005},
  publisher={Elsevier}
}
@article{zamarripa2016rolling,
  title={{Rolling horizon approach for production--distribution coordination of industrial gases supply chains}},
  author={Zamarripa, Miguel and Marchetti, Pablo A and Grossmann, Ignacio E and Singh, Tejinder and Lotero, Irene and Gopalakrishnan, Ajit and Besancon, Brian and Andr{\'e}, Jean},
  journal={Industrial \& Engineering Chemistry Research},
  volume={55},
  number={9},
  pages={2646--2660},
  year={2016},
  publisher={ACS Publications}
}
@article{achkar2024efficient,
  title={Efficient computational strategies for a mathematical programming model for multi-echelon inventory optimization based on the guaranteed-service approach},
  author={Achkar, VG and Brunaud, BB and Musa, Rami and Grossmann, IE},
  journal={Computers \& Chemical Engineering},
  volume={182},
  pages={108567},
  year={2024},
  publisher={Elsevier}
}
@article{eruguz2016comprehensive,
  title={A comprehensive survey of guaranteed-service models for multi-echelon inventory optimization},
  author={Eruguz, Ayse Sena and Sahin, Evren and Jemai, Zied and Dallery, Yves},
  journal={International Journal of Production Economics},
  volume={172},
  pages={110--125},
  year={2016},
  publisher={Elsevier}
}

==> sections/gdp.tex <==
\subsection{Generalized Disjunctive Programming} \label{sec:gdp}

Generalized Disjunctive Programming (GDP) is a mathematical optimization framework that allows modeling and solving problems with disjunctive constraints in a systematic way.
It was first introduced by \citet{raman1994modelling} as extension of the disjunctive programming paradigm proposed by \citet{balas1985disjunctive}, which modeled modeled a feasible region as a disjunction of convex sets. Overall, GDP is a powerful mathematical framework that enables the modeler to integrate algebraic constraints with Boolean logic and disjunctive constraints \citep{grossmann2013systematic}. The general formulation of a GDP is as follows:

\begin{equation}\label{eqn:gdp.general}
\begin{aligned}
\min &\ f(x) \\
s.t. \quad &\ g(x) \leq 0\\
&\ \bigveebar_{i\in D_k} \left[
    \begin{gathered}
    Y_{ik} \\
    r_{ik}(x)\leq 0\\
    \end{gathered}
\right] \quad k \in K\\
&\ \Omega(Y) = \text{True} \\
&\ x \in X \subseteq \mathbb{R}^n\\
&\ Y_{ik} \in \{\text{True}, \text{False}\} \quad k \in K, i \in D_k\\
\end{aligned} 
\end{equation}
which is defined over a set of real variables $x$ specified over a domain $X$, where $f(x)$ is the objective function and $g(x)$ is set of global constraints. In addition, the Boolean variable $Y_{ik}$ serves as an indicator, determining whether to enforce the set of constraints $r_{ik}$, which corresponds to the set of the $i$th disjunct in the $k$th disjunction. Every disjunct is related through an exclusive OR ($\underline{\vee}$), which can be thought of as an $exactlyOne$ operator when $|D_k|>2$, that enforces only one set of constraints per disjunction \citep{perez2023modeling}. $\Omega(Y)$ is the set of logical prepositions composed of clauses relating the Boolean variables through the first order operators AND ($\wedge$), OR ($\vee$), negation ($\neg$), implication ($\Rightarrow$) and equivalence ($\Leftrightarrow$). 

One of the key features of GDP is its ability to model systems based on their underlying logical relationships. 
This approach enables a more intuitive modeling by representing discrete decisions and their relationships in terms of disjunctions and Boolean logic propositions \citep{grossmann2002review,grossmann2013systematic}. This helps avoid common modeling mistakes associated with direct application of  mixed-integer constraints. Similarly, it also provides a clearer representation of complex systems, making the optimization modeling more efficient, reliable and interpretable.

Another important advantage of Generalized Disjunctive Programming is its versatility in solution methods, which can be broadly classified into two categories. The first category encompasses techniques that involve transforming the GDP into a mixed-integer (non)linear program. Methods within this category, such as Big-M \citep{raman1994modelling}, hull \citep{lee2000new}, and hybrid approaches \citep{sawaya2005cutting}, aim to represent the logical structure of the problem within the framework of mixed-integer programming. These methods facilitate the utilization of established optimization solvers. The second category comprises logic-based methods that operate directly within the logical structure of the problem. Approaches like Logic-based Outer Approximation  \citep{turkay1996logic} and Logic-Based Branch-and-Bound \citep{grossmann2002review} fall into this category, leveraging the inherent logical relationships present in the disjunctive structure of the problem. 

In this work, our approach does not solve generalized disjunctive programs directly. Rather than tackling the optimization problems within the GDP framework, our focus lies in utilizing this GDP to articulate disjunctive constraints in an intuitive and interpretable manner through disjunctions. Hence, all posed disjunctions are reformulated into mixed-integer constraints. Notably, for each disjunction, we explicitly and individually propose a reformulation into a set of mixed-integer constraints. For this, we introduce the associated binary variable $y$ as:

\begin{equation}
    \begin{aligned}
    y_{ik} = \mathbbm{1}\{Y_{ik}\} \quad k \in K, i \in D_k \\
    \ y_{ik} \in \{0, 1\} \quad k \in K, i \in D_k\\
\end{aligned}
\end{equation}
to represent the a binary mapping of the Boolean value. We would use the associated binary variables, written as the lower case letter of their Boolean counterpart, to pose the mixed-integer reformulation of all proposed disjunctions. 
